Graph Surfing in Reaction Systems from a Categorial Perspective

Graph-based reaction systems were recently introduced as a generalization of the intensely studied set-based reaction systems. They deal with simple edge-labeled directed graphs, and dynamic semantics of graph-based reaction systems is defined by graph surfing as a novel kind of graph transformation where, in a single surf step, reactions are applied to a subgraph of a given background graph yielding a successor subgraph. In this paper, we propose a categorical approach to reaction systems so that a wider spectrum of data structures becomes available on which reaction systems can be based. In this way, many types of graphs, hypergraphs, and graph-like structures are covered.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{B. Hoffmann and M. Minas (Eds.): Eleventh International\\ 
Workshop on Graph Computation Models (GCM 2020)\\
EPTCS 330, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.330.5}{10.4204/EPTCS.330.5}}
\pdfoutput=1

